Message-Passing Algorithms and Homology

This PhD thesis lays out algebraic and topological structures relevant for the study of probabilistic graphical models. Marginal estimation algorithms are introduced as diffusion equations of the form $\dot u = \delta \varphi$. They generalise the traditional belief propagation (BP) algorithm, and provide an alternative for contrastive divergence (CD) or Markov chain Monte Carlo (MCMC) algorithms, typically involved in estimating a free energy functional and its gradient w.r.t. model parameters. We propose a new homological picture where parameters are a collections of local interaction potentials $(u_\alpha) \in A_0$, for $\alpha$ running over the factor nodes of a given region graph. The boundary operator $\delta$ mapping heat fluxes $(\varphi_{\alpha\beta}) \in A_1$ to a subspace $\delta A_1 \subseteq A_0$ is the discrete analog of a divergence. The total energy $H = \sum_\alpha u_\alpha$ defining the global probability $p = e^{-H} / Z$ is in one-to-one correspondence with a homology class $[u] = u + \delta A_1$ of interaction potentials, so that total energy remains constant when $u$ evolves up to a boundary term $\delta \varphi$. Stationary states of diffusion are shown to lie at the intersection of a homology class of potentials with a non-linear constraint surface enforcing consistency of the local marginals estimates. This picture allows us to precise and complete a proof on the correspondence between stationary states of BP and critical points of a local free energy functional (obtained by Bethe-Kikuchi approximations) and to extend the uniqueness result for acyclic graphs (i.e. trees) to a wider class of hypergraphs. In general, bifurcations of equilibria are related to the spectral singularities of a local diffusion operator, yielding new explicit examples of the degeneracy phenomenon. Work supervised by Pr. Daniel Bennequin

==> II/basespace.tex <==

\subsubsection{Partial Orders.} 

A partial order $(X, \leq)$ in $\Ord$ is a category
with a unique arrow $\aa \aw \bb$ when $\aa \leq \bb$. 
A morphism between $X$ and $Y$ in $\Ord$ is thus a
functor between $X$ and $Y$.

\subsubsection{Hypergraphs.}

A hypergraph on a set $\Om$ is a collection of 
subsets $X \incl \Part(\Om)$. 
A hypergraph $X$ is a partial order. 

\subsubsection{Admissible Decompositions.}

An admissible decomposition of $\Om$ 
is a hypergraph $X \incl \Part(\Om)$:
\bi
\iii closed under intersection:
$\bb \cap \cc  \in X$ for all $\bb, \cc \in X$
\iii with conditional unions: 
$\bb \cup \cc \in X$ if there exists $\aa \in X$ such that $\aa \aw \bb$ and
$\aa \aw \cc$. 
\ei
This defines a subcategory $\Ord'$ of $\Ord$ with obvious morphisms.

\subsubsection{Simplicial Complexes.} 

A simplicial complex $K$ is a hypergraph on 
its set $\Om$ of vertices such that:
\bi
\iii if $\bb \incl \aa$ and $\aa \in K$, then $\bb \in K$.
\ei
An $n$-simplex of $K$ is a set of $n+1$ vertices. 
The set of $n$-simplices of $K$ is denoted by $K_n$.
The dimension of $K$ is the maximal $n$ such that $K_n \neq \vide$. 

N.B. A simplicial complex is an admissible decomposition. 
The category $\KS$ of simplicial complexes is a subcategory of $\Ord'$. 

\subsubsection{Oriented Simplicial Complexes.} 

An orientation of a simplicial complex $K$ 
is a collection of total orders on each simplex, such that
for every $\aa \aw \bb$ in $K$,
the order induced by $\aa$ on $\bb$ is consistent
with that of $\bb$. 
Denote by $\KS^+$ the category of oriented simplicial complexes. 

\subsubsection{Nerve.}

Given a partial order $X$ in $\Ord$, 
its nerve is the oriented simplicial complex $NX \incl \Part(X)$
whose $p$-simplices are the non-degenerate $p$-chains of $X$:
\begin{equation} N_p X = 
\{ \aa_0 \aw \dots \aw \aa_p \in X  \st i \neq j \impq \aa_i \neq \aa_j \} \end{equation}
The nerve defines a functor $N : \Ord \aw \KS^+$.



==> II/fields.tex <==
\subsection{Observables}

An observable on a region $\aa \incl \Om$ is a real function 
on $E_\aa$, we denote by $\obs_\aa = \R^{E_\aa}$ the commutative algebra
of observables on $\aa$. 
For every subregion $\bb \incl \aa$, any observable $u_\bb \in \obs_\bb$
admits a cylindrical extension,
$j_{\aa\bb}(u_\bb) \in \obs_\aa$ defined by pulling back
the projection of $E_\aa$ onto $E_\bb$:
\begin{equation} j_{\aa\bb}(u_\bb) = u_\bb \circ \pi^{\bb\aa} \end{equation}
The injections $j_{\aa\bb}$ make $\obs:X^{op} \aw \Alg$
a contravariant functor to the category of unital real algebras.
We denote by $1_\aa$ the unit of $\obs_\aa$ and 
will generally drop the injection in our notation.  

We call observable field an allocation of observables on the nerve of $X$,
defining an observable on a $p$-chain $\bar\aa \in N^p X$ 
to be an observable on its smallest region $\aa_p$. 
We write $\obs_{\bar \aa}$ for the copy of $\obs_{\aa_p}$ on  $\bar \aa$,
and denote the space of $p$-fields by:
\begin{equation} \obs_p(X) = \bigoplus_{\bar \aa \in N^p X} \obs_{\bar \aa} \end{equation}
and by $\obs(X)$ the graded vector space of observable fields.
If $\bar \bb$ is a face of $\bar \aa$, its terminal region contains that
of $\bar \aa$. 
It follows that there is a canonical injection 
$j_{\bar \bb \bar \aa} : \obs_{\bar \aa} \aw \obs_{\bar \bb}$ whenever
$\bar \bb$ is a subchain of $\bar \aa$.\footnote{
    Observable fields form a simplicial algebra 
    $\obs(X) : \Ord^{op} \aw \Alg$. 
    Our construction is related to this more 
    general theory,
    see Segal's note on classifying spaces \cite{Segal-68} for instance.
}

The boundary operator $\div : \obs_{p+1}(X) \aw \obs_p(X)$
 is defined on a $(p+1)$-field $\ph$ by the following formula:
\begin{equation} (\div \ph)_{\bar \bb}  = \sum_{k=0}^{p+1} \,
\sum_{\div_k \bar \aa' = \bar \bb} (-1)^k \, j_{\bar \bb \bar \aa'}(\ph_{\bar \aa'}) \end{equation}
The proof of $\div^2 = 0$ is done as usual, 
it uses functoriality of the injections but otherwise does not differ from
the case of scalar coefficients.
In the case where $p = 0$, we have for example:
\begin{equation} \div_\bb \ph = \sum_{\aa' \aw \bb} \ph_{\aa'\bb} 
- \sum_{\bb \aw \cc'} \ph_{\bb \cc'} \end{equation}

Each $\obs_\aa$ 
may also be viewed as the abelian Lie algebra of the multiplicative
Lie group 
$G_\aa = (\R_+^*)^{E_\aa}$
of strictly positive observables on $\aa$.
We denote by: 
\begin{equation} \expm_\aa : \obs_\aa \aw G_\aa \end{equation}
the group isomorphism $u_\aa \mapsto \e^{-u_\aa}$ 
and by $\mlog_\aa$ its inverse.

\subsection{Measures.}

We call density on a region $\aa \incl \Om$ a linear form on observables 
$\om_\aa \in \obs^*_\aa$. For every $\bb \incl \aa$, we denote 
by $\Sigma^{\bb\aa}(\om_\aa) \in \obs^*_\bb$ the density defined 
by integrating $\om_\aa$ along the fibers of $\pi^{\bb\aa}$:
\begin{equation} \Sigma^{\bb \aa}(\omega_\aa)(x_\bb) = 
\sum_{x' \in E_{\aa \setminus \bb}} \omega_\aa(x_\bb, x') \end{equation}
The marginal projections $\Sigma^{\bb\aa}$ make $\obs^* : X \aw \Vect$
a covariant functor. 
Each $\Sigma^{\bb\aa}$ is
dual to $j_{\aa\bb}$ as 
for every $\omega_\aa \in \obs^*_\aa$ and every $u_\bb \in \obs_\bb$, 
we have:
\begin{equation} \croc{\Sigma^{\bb \aa}(\omega_\aa)}{u_\bb} 
= \croc{\omega_\aa}{j_{\aa\bb}(u_\bb)} \end{equation}

We define the complex $\obs^*(X)$ of density fields
by duality with $\obs(X)$, 
and denote its differential by $\diff$, adjoint of $\div$. 
The action of $\diff$ on a density $p$-field $\omega$ 
is the $(p+1)$-field defined by:
\begin{equation} (\diff \omega)_{\bar \aa} = \sum_{k = 0}^p (-1)^k \, 
\Sigma^{\bar \aa \, \div_k \bar \aa}(\omega_{\div_k \bar \aa}) \end{equation}
writing $\Sigma^{\bar \aa \bar \bb}$ for the adjoint of $j_{\bar \bb \bar \aa}$.
For $p = 0$, we have:
\begin{equation} (\diff \omega)_{\aa \bb} = \omega_\bb - \Sigma^{\bb \aa}(\omega_\aa) \end{equation}
We say that a field $\omega \in \obs^*_0(X)$ is consistent if 
$d\om = 0$. 
For every region $\aa \in X$ and
every subregion $\bb \incl \aa$, the marginal
of $\omega_\aa$ on $\bb$ is then $\omega_\bb$.

A density $\om_\aa$ on $\aa$ is said positive if $\om_\aa(u^2_\aa) \geq 0$
for every observable $u_\aa$.
The counting measure on $E_\aa$, denoted by $1^\flat_\aa$,
is positive. Its free orbit under multiplication by the observables of $G_\aa$
is the space of strictly positive densities, 
we will sometimes identify $G_\aa$ with $G_\aa \cdot 1^\flat_\aa \incl \obs^*_\aa$.

\subsection{Statistical States}

A statistical state on a region $\aa \incl \Om$ is a positive 
density $p_\aa \in \obs^*_\aa$ such that $p_\aa(1_\aa) = 1$.
Equivalently, it is a probability measure on $E_\aa$ and 
we denote by $\Delta_\aa = \Prob(E_\aa)$ the convex set of 
statistical states on $\aa$.
It is a topological simplex of dimension $|E_\aa| - 1$ 
and its image under $\Sigma^{\bb\aa}$ is $\Delta_\bb$, so that
$\Delta : X \aw \Top$ defines a covariant functor of topological spaces.
Any non-trivial positive density $\om_\aa \in \obs^*_\aa$ defines a
normalised statistical state which we denote by $[\om_\aa] \in \Delta_\aa$.

The interior $\Del_\aa$ of the probability simplex on $E_\aa$
consists of all the non-vanishing probability densities. 
It is diffeomorphic to the quotient of $G_\aa$ by scalings of $\R_+^*$,
itself isomorphic to the quotient of $\obs_\aa$ by the action of additive constants:
\begin{equation} \Del_\aa \sim \P G_\aa \sim \obs_\aa / \R \end{equation}
It follows that $\Del_\aa$ has a natural Lie group structure.
The extensions $j_{\aa\bb}$ admit a quotient by scalings
and $\Del : X^{op} \aw \Grp$ also defines a contravariant functor.
The Gibbs state associated to any observable $U_\aa \in \obs_\aa$ 
is the non-vanishing probability density $[\e^{-U_\aa}] \in \Del_\aa$
and we denote by:
\begin{equation} \gibbs_\aa : G_\aa \aw \Del_\aa \end{equation}
the surjective group morphism induced by Gibbs states.

The convex set $\Delta(X) \incl \obs^*(X)$ of statistical fields 
may be defined by inclusion of each $\Delta_\aa \incl \obs^*_\aa$
and we denote by $\Del(X)$ the interior of $\Delta(X)$. 
We say that $p \in \Delta(X)$ is a consistent statistical field if $dp = 0$ 
and denote by $\Zp \incl \Del_0(X)$ 
the subset of non-vanishing consistent statistical fields.


\begin{comment}
\subsection{Simplicial Groups.}


% this relevant || just redirect ?
Before proceeding to explicit constructions,
we only wish to point out the fact that they may be related to 
the more general theory of simplicial groups.
We provide a mere reference here and
kindly redirect the interested reader to [Segal, Orsted].

Let $\Ord$ denote the category of finite totally ordered sets
with order preserving functions as morphisms.
For any $n \in \N$ we denote by $[n]$ the object $\{ 0, \dots, n \}$.
We denote by $\div_i : [n-1] \aw [n]$ the $i$-th face map, 
whose image misses the $i$-th element of $[n]$.

A simplicial object $K$ in a category $\mathbf C$ is a contravariant functor 
$K : \Ord^{op} \aw \mathbf C$.
The nerve of $X$ is an example of simplicial set, 
whose $p$-simplices are the elements of $N^p X = NX([p])$. 
A simplicial abelian group $K : \Ord^{op} \aw \Ab$ 
yields a chain complex with boundary $\div : K([n]) \aw K([n-1])$ 
defined by: 
\begin{equation} \div = \sum_{i = 0}^{n} (-1)^i K(\div_i) \end{equation}
The dual notion of cosimplicial abelian group $K': \Ord \aw \Ab$
yields a cochain complex.
\end{comment}



==> II/homology.tex <==

We prove the acyclicity of the whole complex by building  
a homotopy retracting $A_\bullet(X)$ 
on $A_0(X)$. 
For every $\aa \in X$ and $n \geq 1$, consider the map
$e_\aa : A_n(X) \aw A_{n+1}(X)$ 
defined by: 
\begin{equation} e_\aa(\ph)_{\aa' \bar \bb} = 
\left\{ \ba{ll}
\ph_{\bar \bb} &\txt{if} \aa' = \aa \\
0   &\txt{otherwise}
\ea \right. \end{equation}
Anticipating 
on the next chapter,
let us assume there exists a collection of integers $(c_\aa) \in \Z_0(X)$ 
such that for all $\bb \in X$: 
\begin{equation} \sum_{\aa \cont \bb} c_\aa = 1 \end{equation}
We will show that the homotopy
$\eta = \sum_\aa c_\aa \cdot e_\aa$ defines a retraction on $A_0(X)$.


\begin{lemma} 
    For every $\aa \in X$, we have:
    \begin{equation} \div e_\aa + e_\aa \div = {\bf 1}_{\LL^\aa} - \zeta_\aa \end{equation}
    where $\zeta_\aa : A_\bullet(X) \aw A_0(X)$ is the homogeneous map defined by: 
    \begin{equation} \zeta_\aa(u) = \sum_{\aa \aw \bb} u_\bb \end{equation}
    and ${\bf 1}_{\LL^\aa}$ denotes the canonical projection of 
    $A_\bullet(X)$ onto $A_\bullet(\LL^\aa)$. 
\end{lemma}

\begin{proof}
%    \begin{equation} \div (e_\aa \ph)_{\bb \bar \cc} = 
%    (e_{\aa} \ph)_{\aa \bb \bar \cc} - 
%    \sum_{p = 0}^{n+1} \end{equation}
    The proof amounts to a simple computation and s
    For every $\ph \in A_n(X)$ and $\bar \bb = \bb \bar \cc \in N_n(X)$ 
    let us adopt the following notation:
\begin{equation} e_\aa(\div \ph)_{\bb \bar \cc} = 
    {\bf 1}_{[\aa = \bb]} \cdot \div_{\bar \cc} \ph \end{equation}
    the above vanishing when $n = 0$.
On the other hand, we have:
    \begin{equation} \div(e_\aa \ph)_{\bar \bb} = (e_\aa \ph)_{\aa \bar \bb} 
    + \sum_{p = 1}^{|\bar \bb| + 1} 
    (-1)^p \sum_{\div_p \bar \aa' = \bar \bb} (e_\aa \ph)_{\bar \aa'} \end{equation}
    and writing the summation variable as $\bar \aa' = \bb \bar \bb'$ 
    we get:
    \begin{equation} \begin{split} 
        \div(e_\aa \ph)_{\bar \bb} 
        &= \ph_{\bar \bb} - 
        \sum_{k = 0}^{|\bar \cc| + 1} (-1)^k \sum_{\dr_k \bar \bb' = \bar \cc} 
        (e_\aa \ph)_{\bb \bar \bb'} \\
    &=  
    \ph_{\bar \bb} - {\bf 1}_{[\aa = \bb]} \cdot \div_{\bar \cc} \ph
    \end{split} \end{equation}
    the last line holding only when $n \geq 1$, otherwise we have:
    \begin{equation} \div(e_\aa u)_\bb = u_\bb - {\bf 1}_{[\aa = \bb]} \sum_{\aa \aw \bb'} 
    u_{\bb'} \end{equation}
    for every $u \in A_0(X)$ and $\bb \in X$.
\end{proof}

\begin{thm} 
    The map $\eta : A_\bullet(X) \aw A_{\bullet+1}(X)$ defined by:
    \begin{equation} \eta = \sum_{\aa \in X} c_\aa \cdot e_\aa \end{equation}
    defines a homotopy retracting $A_\bullet(X)$ on $A_0(X)$: 
    \begin{equation} \eta \div + \div \eta = 1 - C \end{equation} 
    where $C : A_\bullet(X) \aw A_0(X)$ is the homogeneous map
    defined by:
    \begin{equation} C(u)_\aa = c_\aa \sum_{\aa \aw \bb} u_\bb \end{equation}
\end{thm}

\begin{proof} 
    This is an easy consequence of the lemma, since
    \begin{equation} \sum_{\aa \in X} c_\aa \cdot {\bf 1}_{\LL^\aa} = {\bf 1} \end{equation}
\end{proof}

\begin{comment}
\begin{thm} 
    The degree $1$ endomorphism of $A_\bullet(X)$ defined 
    for every $\ph \in A_p(X)$ and $\bar \aa \in N_p(X)$ by:
    \begin{equation} \eta(\ph)_{\bar \aa \bb} = (-1)^{p+1}\, P^{\bb \bar \aa}(\ph_{\bar \aa}) \end{equation}
    is a homotopy between $P : A_\bullet(X) \aw Z_0(X)$ and the 
    identity of $A_\bullet(X)$: 
    \begin{equation} \eta \div + \div \eta = 1 - P \end{equation}
    hence $A_\bullet(X)$ is acyclic and $H_\bullet(X) = Z_0(X)$.
\end{thm}
\end{comment}


==> IV/ii_diffusion.tex <==
\subsection{Diffusion}

\subsubsection{Decompositions.}

Let us denote by $H_\Omega$ the hamiltonian of a statistical system $\Omega$.
It may be thought of as an observable on $\Omega$, at least 
until one is faced with the problem that $\Omega$
is hardly observable\footnotemark{}. 
We still denote by $\obs_\Omega$ the space of observables on $\Omega$ 
although we should think of it as abstractly as possible.

\footnotetext{
Physics of phase transitions require to study the limit of arbitrarily 
large $\Omega$ where the mean value of extensive observables diverge.
Computational methods are soon faced with untractable datasets.
}

A decomposition $X$ of $\Omega$ will be said adapted\footnote{
cf. GSP: minimal $X$
} 
to $H_\Omega$ if there exists a field of local energies
$h \in \obs_0(X)$ decomposing $H_\Omega$ in $\obs_\Omega$:
\begin{equation} H_\Omega = \sum_{\aa \in X} h_\aa \end{equation} 
Reciprocally, let us denote by $\obs_X$ the inductive limit of $\obs$ over $X$.
Writing $\zeta_\Omega$ for the canonical projection: 
\begin{equation} \zeta_\Omega : \obs_0(X) \aw \obs_X \end{equation}
we call $\zeta_\Omega(h) = H_\Omega$ the global sum of $h$.

More generally, given a field of local potentials $h \in \obs_0(X)$,
we define the internal hamiltonian $H_\aa$ of a region $\aa$ to be:
\begin{equation} H_\aa = \sum_{\bb' \in \Lambda^\aa} h_{\bb'}  \end{equation}
We similarly write $\zeta_\aa(h) = H_\aa$
as this is the left action of $\zeta \in \tilde\R_1(X)$ 
on $h$.
The two fields $H$ and $h$ are in bijective correspondence,
we call $H = \zeta \cdot h$ the local sums 
of $h$ and $h = \mu \cdot H$ the local decomposition of $H$. 

The internal hamiltonians usually account for the state
of each subsystem had it been isolated, 
while only the global hamiltonian describes the actual state of the total system.
In this sense it is natural to treat all the possible decompositons of $H_\Omega$ 
We shall see that $H_\Omega$ actually describes 
the homology class of $h$ in $H_0(\obs(X), \div)$ 
and denote by ${\cal D}(H_\Omega)$ the subspace of its decompositions.

\subsubsection{Effective Gradient.}

We introduce non-linear functionals from $\obs_0(X)$ to $\obs_1(X)$
that will transport energy between the subsystems of $\Omega$,
each region receiving an effective energy flux that should account
for its interaction with the rest of the system. 

Given $H \in \obs_0(X)$, 
we first introduce the field $\nabF(H) \in \obs_1(X)$ defined by:
\begin{equation} \nabF(H)_{\aa\bb} = H_\bb - \Fh^{\bb\aa}(H_\aa) \end{equation}
and call $\nabF(H)$ the effective gradient of $H$.
Denoting by $h = \mu \cdot H$ the local decomposition of $H$, 
we also consider the field $\Phi(h) \in \obs_1(X)$ defined by:
\begin{equation} \Phi_{\aa\bb}(h) = \Fh^{\bb\aa}
\bigg(  \sum_{\bb' \in \Lambda^\aa \setminus \Lambda^\bb} h_{\bb'} 
\bigg) \end{equation}
which is the effective contribution of $\Lambda^\aa \setminus \Lambda^\bb$
to the energy of $\Lambda^\bb$. These two functionals are related by:
\begin{equation} \Phi = - \nabF \circ \zeta \end{equation}

We say that $U$ is an effective cocycle when $\nabF(U) = 0$
and we denote by $\ZU \incl \obs_0(X)$ the set of effective cocycles.
We say that $u$ is an effective potential if $U = \zeta \cdot u$ 
is an effective cocycle, and denote by $\Zu = \mu \cdot \ZU$ the
set of effective potentials. 

The local Gibbs states of any effective cocycle $U \in \ZU$
define a consistent statistical field $\rho \in \Zp$.
However, a field of effective hamiltonians $U$ 
also induces a consistent statistical field if its
effective gradient $\nabF(U) \in \R_1(X)$ is a scalar field, 
so the condition $U \in \ZU$ is strictly stronger than 
$\rho \in \Zp$.

\subsubsection{Transport.}

Suppose given a field of local potentials $h \in \obs_0(X)$ decomposing
the global hamiltonian $H_\Omega$, and an energy flux $\ph \in \obs_1(X)$.
We consider the transport of $h$ by $\ph$ and 
as the field of local potentials $u \in \obs_0(X)$ defined by:
\begin{equation} u = h + \div \ph \end{equation}
The effect of $\ph$ consists of moving energy terms 
around $X$ and does not affect their global sum, 
but we will also be interested in the variations 
of the local sums $U = \zeta \cdot u$ and $H = \zeta \cdot h$.

More precisely, consider the transport equation:
\begin{equation} \dot u = \div \Phi(u) \end{equation}
and denote 
by $\Xi = \div \Phi$ the induced vector field on $\obs_0(X)$.
We take $u(0) = h$ as initial condition, so that $u(t)$ is always homologous
to $h$. A slightly different point of view is to define the potentials by
$u = h + \div \ph$ and the dynamics by
$\dot \ph = \Phi(h + \div \ph)$.
We may denote by $\Xi'$ the induced vector flow on $\obs_1(X)$, 
with $\div \Xi' = \Xi$.

In absence of normalisation\footnote{
    This is the case of the original algorithm on trees as introduced by Pearl.
}
Belief Propagation 
is the naive Euler scheme 
approximating the flow of $\Xi$ by: 
\begin{equation} \e^{n \tau \Xi} \simeq (1 + \tau \Xi)^n \end{equation}
Note that BP is actually for $\tau = 1$ 
and the choice of a time scale would appear as exponents in 
the multiplicative formulation.
BP is usually viewed as an algorithm on messages, 
which is the Euler scheme for $\Xi'$.


For every region $\aa \in X$, let us define the coboundary 
of the subsystem $\Lambda^\aa$ as the subset of arrows 
$\cobord{\aa} \incl N^1 X$ that meet $\Lambda^\aa$ but  
are not contained in $\Lambda^\aa$: 
\begin{equation} \cobord{\aa} = 
\{ \aa' \aw \bb' \st \aa' \not\in \Lambda^\aa \txt{and} \bb' \in \Lambda^\aa \}
\end{equation}
The following proposition may then be thought of as a Gauss formula on $\Lambda^\aa$: 

\begin{prop}
    For every $\ph \in \obs_1(X)$ and $\aa \in X$ we have:
    \begin{equation} \sum_{\bb' \in \Lambda^\aa} \div_{\bb'} \ph = 
    \sum_{\aa'\bb' \in \cobord{\aa}} \ph_{\aa'\bb'} \end{equation}
    In particular, the above vanishes if $\ph$
    is supported in $\Lambda^\aa$.
\end{prop}

\begin{proof} In the sum of $\div \ph$ over $\Lambda^\aa$, 
each term $\ph_{\bb\cc}$ appears with opposite signs 
in $\div_{\bb}\ph$ and $\div_{\cc} \ph$ 
whenever both $\bb$ and $\cc$ belong to $\Lambda^\aa$.
\end{proof}



* * *

{\it Remark.} Why not instead consider the flux $\Psi$ defined by:
\begin{equation} \Psi_{\aa\bb} = \sum_{\cc' \in \Lambda^\bb} \mu_{\bb\cc'} \Phi_{\aa\cc'} \end{equation}
On a graph, $\Phi = \Psi \mod \R$ as the depth of $X \setminus \{ \vide \}$ is one.
This flow should have better convergence properties 
as $\zeta_\aa(\div \Psi)$ only counts once each term of the form 
$\Fh^{\bb\aa'}(U_{\aa'})$, where $\bb = \aa \cap \aa'$.

 * * *

\begin{thm}
Let $h \in \obs_0(X)$ be a decomposition of $H_\Omega$.
The space of decompositions $\Dec(H_\Omega)$ 
is the homology class of $h$ for $\div$: 
    \begin{equation} u \in \Dec(H_\Omega) \eqvl u \in h + \Img(\div) \end{equation}
\end{thm}

\begin{proof}
Requires the interaction decomposition $\obs_\aa = \bigoplus_\bb \z_\bb$.
\begin{itemize}
        \iii $\Img(\div) \incl \Dec(0)$: consequence of Gauss formula.
        \iii $\Dec(0) \incl \Img(\div)$: define $\ph_{\aa\bb} = P_\bb(h_\aa)$ 
        and check that $(h + \div \ph)_\bb = P_\bb(H_\Omega)$. 
\end{itemize}

\end{proof}


==> TODO <==
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
------
./VI/i/cocyclic.tex-  44-	yields $U + \zeta \cdot \div \ph = V$. 
./VI/i/cocyclic.tex:  45:	[[ $T_\aa$ via one-step iteration of 5.3.2 ]]
./VI/i/cocyclic.tex-  46-
--
./VI/i/cocyclic.tex-  51-	local hamiltonians, 
./VI/i/cocyclic.tex:  52:	the Gauss formula \ref{zeta-cocycle} [[Gauss 2.2.2]] 
./VI/i/cocyclic.tex-  53-	implies $U_\aa = V_\aa$ while consistency 
------
------
------
------
------
------
------
------
./VI/iii/laplacian.tex- 129-	    then $\det_\C(g_*)$ would also vanish on an open subset in $M_\C$,
./VI/iii/laplacian.tex: 130:	    hence everywhere by analytic continuation [[why go to $\C$?]]. 
./VI/iii/laplacian.tex- 131-	    As this would violate Sard's theorem, it follows that 
------
------
./VI/iii/graphs.tex-   63-
./VI/iii/graphs.tex:   64:	[[fig. Kirchhoff and $E, C, L$]]
./VI/iii/graphs.tex-   65-
--
./VI/iii/graphs.tex-  132-	of parameters, the real largest eigenvalue of $\M$ has to cross $1$. 
./VI/iii/graphs.tex:  133:	This approach proved the existence of at least [[six bifurcations]] 
./VI/iii/graphs.tex-  134-	on the simple "figure eight". 
--
./VI/iii/graphs.tex-  245-
./VI/iii/graphs.tex:  246:	[[fig. triangle-edge]]
./VI/iii/graphs.tex-  247-
------
./VI/iii/transversality.tex-   1-
./VI/iii/transversality.tex:   2:	[[Define $\nabla$ or move to 5.2.1]]
./VI/iii/transversality.tex-   3-	At the level of local hamiltonians, 
--
./VI/iii/transversality.tex-  13-	Let us denote by $\bar 0 = \mu \cdot \ln [1]$ the {\it origin} of $\Z$, 
./VI/iii/transversality.tex:  14:	projection of $0 \in \Z'$ onto $\Z$ along $\R_0$, as defined in [[5.2.1]].
./VI/iii/transversality.tex-  15-
--
./VI/iii/transversality.tex-  31-	in $T_{\bar 0}{\cal Z}$ homologous to $u \in A_0$. 
./VI/iii/transversality.tex:  32:	The map $P : u \mapsto v$ coincides with the interaction projection of [[2.3.3]].
./VI/iii/transversality.tex-  33-	\end{proof}
--
./VI/iii/transversality.tex-  60-	\begin{proof}
./VI/iii/transversality.tex:  61:	- [[2.3.3]] In $A_0$ we have $\Ker(d) = \zeta \cdot Z_0$. 
./VI/iii/transversality.tex-  62-	The change of  metric is simply reflected by conjugating 
--
./VI/iii/transversality.tex-  65-	Hence $\Ker(\nabla) = p^{-1} \cdot \Ker(d)$, while 
./VI/iii/transversality.tex:  66:	by definition [[5.2.1]] of $\nabla$ we have 
./VI/iii/transversality.tex-  67-	$T_u {\cal Z} = \Ker(\nabla \circ \zeta)
------
------
------
------
------
------
------
------
./V/diffusion.tex-   27-
./V/diffusion.tex:   28:	[[Tangent map $\nabla = \DF_*$]]
./V/diffusion.tex-   29-	\begin{prop} 
--
./V/diffusion.tex-  155-	    if and only if there exists Lagrange multipliers $\ph$ such that 
./V/diffusion.tex:  156:	    $- \ln(q) = H + \zeta \cdot \bord' \ph$ [[in virtue of theorem 4.X]].
./V/diffusion.tex-  157-	    \bi
------
------
------
------
------
------
------
./I/lim.tex- 113-
./I/lim.tex: 114:	    \item in some abelian category e.g. $\Vect$ [[Kernel and Image]].
./I/lim.tex- 115-	\end{enumerate}
------
------
------
------
./I/I.tex-  84-	with more elaborate ones, such as inductive and projective limits. 
./I/I.tex:  85:	[[cf Dwyer-Spalinski \cite{Dwyer-Spalinski}, H. Cartan]] 
./I/I.tex-  86-
------
------
./I/nat.tex-  30-	{\bf Examples:}
./I/nat.tex:  31:	[[ $\Hom(-,X)$ and Yoneda ]]
./I/nat.tex:  32:	[[ adjunction example ]]
------
------
------
------
./I/obj.tex-  91-
./I/obj.tex:  92:	[[Define $\Cat^{op}$ ]]
./I/obj.tex-  93-
------
------


==> V/intro.tex <==

\begin{comment}

This algorithm differs slightly from the Generalized Belief Propagation
introduced by Yedidia {\it et al.} in [Yed 2000] but its fixed points 
are also in one-to-one correspondence with the critical points of Bethe free energy.

* * * 

This theoretical definition of equilibrium is hardly computable in practice.
Computational methods are quickly faced with an exponential growth in complexity
with the cardinal of $\O$.
Physics of phase transitions require to study the limit of arbitrary large
$\Omega$, where the mean value of an extensive observable such as $H_\Om$ is 
no longer defined. 


A fixed point of BP is such that:
\begin{equation} q_\bb = \Sigma^{\bb\aa} (q_\aa) \end{equation}

The set of regions $X$ carries structural information about the variables
of $E_\Omega$,  
as for any two regions $\aa$ and $\aa'$ 
the variables of $E_\aa$ and $E_{\aa'}$ should be conditionally independent given 
$E_{\aa \cap \aa'}$.
However the beliefs on $\aa$ and $\aa'$ might not agree on $\aa \cap \aa'$
and one should not rely on a probabilistic interpretation of beliefs.
\end{comment}


==> VI/_global.tex <==
\begin{defn}
Given $\Om = \aa \sqcup_{\bb} \aa'$,
assume $X = \LL^\aa \sqcup_{\LL^\bb} \LL^{\aa'}$ and let 
$\tilde X = X \sqcup \{ \Om \}$. 
The subsheaf $\Shf(\tilde X) \incl A(\tilde X)$ will be said {\rm retractable} if: 
\begin{equation} \Shf(\tilde X) \cap A(X) \simeq \Shf(X) \end{equation}
\end{defn}

\begin{prop} 
The subsheaf 
${\cal Z}(\tilde X) = \{ u \in A_0(\tilde X) \st \DF(\zeta \cdot u) = 0 \}$
is retractable. 
\end{prop}

\begin{proof}
Given $u \in A_0(X)$ and letting $U = \zeta \cdot u$, 
we have $u \in \Shf(\tilde X)$ if and only if:
\begin{equation} \DF(U)_{\Om \aw \aa}  = 0 \txt{and}
\DF(U)_{\Om \aw \aa'} = 0 \txt{and}
\DF(U)_{|X} = 0 \end{equation}
As $\Om \setminus \aa = \aa' \setminus \bb$ 
and $X = \LL^\aa \sqcup_{\LL^\bb} \LL^{\aa'}$, 
by propositions \ref{eff-indep} and \ref{eff-add}, we have for all 
$U = \zeta \cdot u \in A_0(X)$:
\begin{equation} \DF(U)_{\Om \aw \aa}  
= \: \Fh^{\aa\Om}\bigg( \sum_{\cc' \not\incl \aa} u_{\cc'} \bigg)  
= \:\Fh^{\bb\aa'}\bigg( 
    \sum_{\cc' \in \LL^{\aa'} \setminus \LL^{\bb}} u_{\cc'} \bigg) 
= \DF(U)_{\aa' \aw \bb}
\end{equation}
Interverting the roles played by $\aa$ and $\aa'$, 
we similarly get $\DF(U)_{\Om \aw \aa'} = \DF(U)_{\aa \aw \bb}$
and it follows that 
$\DF(U) = 0$ is equivalent to $\DF(U)_{|X} = 0$ 
for all $U \in \zeta \cdot A_0(X)$. 
The image of $\Shf(X)$ in $A_0(\tilde X)$ by the natural injection 
of $A_0(X)$ into $A_0(\tilde X)$ hence coincides with the intersection 
of $\Shf(\tilde X)$ with $A_0(X)$.
\end{proof}

\begin{thm}
If $X \incl \Part(\Om)$ is retractable, $\tilde X = X \cup \{ \Om \}$,
and $\Shf(\tilde X) \incl A(\tilde X)$ is a retractable subsheaf, 
then for every $u \in A(X)$ the unique $v = u + \div \ph \in \Shf(X)$ 
with $\ph \in A(X)$ 
coincides with the restriction of the unique 
$\tilde v = u + \div \tilde \ph \in \Shf(\tilde X)$.
\end{thm}

\begin{proof}
Reasoning by induction on the length of $X$, 
the statement is tautological when $X = \tilde X = \LL^\Om$. 
Assume now that $X = \LL^\aa \sqcup_{\LL^\bb} X'$ 
with $X' \incl \Part(\Om')$ and $\tilde X' = X' \cup \{ \Om' \}$,
and that $\Shf(\tilde X') \cap A(X')$ coincides with $\Shf(X')$. 

Letting $Y = X \cup \{ \Om' \} = \LL^\aa \sqcup_{\LL^\bb} \LL^{\Om'}$ 
and $\tilde Y = Y \cup \{ \Om \}$,
by retractability we have: 
    \begin{equation} \Shf(\tilde Y)  \cap A(Y) = \Shf(Y) 
    = \Shf(\LL^\aa) \sqcup_{\Shf(\LL^\bb)} \Shf(\LL^{\Om'}) \end{equation}
So that by induction hypothesis: 
    \begin{equation} \Shf(\tilde Y) \cap A(X) 
    = \Shf(\LL^\aa) \sqcup_{\Shf(\LL^\bb)} \big( \Shf(\tilde X') \cap A(X') \big)
    = \Shf(\LL^\aa) \sqcup_{\Shf(\LL^\bb)} \Shf(X') 
    = \Shf(X) 
    \end{equation}
    Showing that $\Shf(\tilde Y)$ actually coincides $\Shf(\tilde X)$ 
    amounts to factorising the limit through $\Om'$ by induction hypothesis. 
    The problem is that $\Shf(\tilde Y)$ is not actually well defined as 
    $\Om' \not\in  \tilde X$...
    Sheaf notion should be made more explicit.
    Restriction maps, etc. 
    They are trivial when inclusions are open with respect to the 
    Alexandrov topology, otherwise involve conjugation with zeta-mu transforms. 
\end{proof}



==> VI/cone.tex <==
\subsection{Conical loop}




==> VII/I.tex <==
\section{Applications}

Factor graphs $\eqvl$ hypergraphs describe the structure of a Markov random field:
\begin{equation} p_\Om(x_\Om) = \frac{1}{Z_\Om} \prod_{\aa \incl \Om} f_\aa(x_\aa) \end{equation}
Two collections of factors $(f_\aa) \sim (f'_\aa)$ are said 
{\it homologous} when $\prod_\aa f_\aa \simeq \prod_\aa f'_\aa$ 
up to a scaling factor,
{\it i.e.} they both provide a factorisation of the same global probability
distribution $p_\Om$. 
The normalisation factor $Z_\Om$ being intractable, the strategy of $\BP$ 
is to approximate the marginals $(p_\aa)$ of $p_\Om$ by finding a collection 
of beliefs $(q_\aa) \sim (f_\aa)$ satisfying the {\it consistency} condition: 
\begin{equation} q_\bb(x_\bb) = \sum_{y \in E_{\aa \setminus \bb}} q_\aa(x_\bb, y) \end{equation}
with $p_\Om \simeq \prod_\aa q_\aa$ up to scaling from the homological condition.

\subsection{Parameter Estimation} 

Maximise over parameters $h$ the log-likelihood of observed data $\bar x$: 
\begin{equation} {\cal L}(\bar x, h) = \frac{1}{N} \sum_{i = 1}^N \log 
p(x^{(i)} \st h) \end{equation}
For fully observed models $\bar x = \bar x_\Om$ and a parametrisation 
$p_\Om \simeq \prod_\aa \e^{-h_\aa}$ the log-likelihood is given by:
\begin{equation} {\cal L}(\bar x, h) = - \sum_\aa \bar \E^\aa[h_\aa] 
- \log Z_\Om(h) \end{equation}
where $\bar \E^\aa$ denotes expectation with respect to the empirical marginal. 
Letting $H_\Om = \sum_\aa h_\aa$ denote the global hamiltonian and 
$\Fh^\Om(H_\Om) = - \log \sum \e^{-H_\Om}$ denote the total free energy, 
the log-likelihood rewrites: 
${\cal L}(\bar x, h) = \Fh^\Om(H_\Om) - \bar \E^\Om[H_\Om]$.
Its variations are given by:
\begin{equation} \der{\cal L}{h_\aa} = p_\aa - \bar p_\aa \end{equation} 
Denoting by $p_\aa = \Sigma^{\aa\Om} \e^{-H_\Om}$ the model marginal 
and by $\bar p_\aa$ the empirical marginal. 
Belief propagation allows to estimate $p_\aa$ to perform gradient ascent on $\cal L$.

\subsection{Structured Prediction} 

Restricted Boltzmann machine with variables decomposed as
$\Om = \Om_v \sqcap \Om_h \sqcap \Om_x$ 









==> intro/II.tex <==
\input{intro/general.tex}

%\section*{Conservation and Consistency}

\input{intro/gibbs.tex}

\begin{comment}
    \section*{From Crystals to Neural Networks}

    \input{intro/crystals.tex}

    \section*{Learning Model Parameters} 

    \input{intro/learning.tex}
\end{comment}

{\color{white} ...}
\newpage
\input{intro/content.tex}




==> intro/content.tex <==
\section*{Outline}

Out of the six chapters contained in this thesis, 
chapters 1 to 3 review and develop the algebraic theory 
we shall rely upon. Non-linear functionals from thermodynamics 
and information geometry are introduced in chapter 4.
Message-passing algorithms are adressed in chapter 5 
and the geometry of their equilibria studied in chapter 6. 
Our final transport equation $\dot u = \div \Phi(u)$ with 
flux $\Phi(u) = -  \mu \circ \DF \circ \zeta \, (u)$
decomposes their dynamic into the following elementary operations:
\bi
\iii $\zeta : A_0(X) \aw A_0(X)$ 
is the zeta transform $\zeta(u)_\aa = \sum_{\aa \cont \bb} u_\bb$
defining  local hamiltonians from interaction potentials. 
Its combinatorial and homological properties are studied in chapter 3.
\iii $\DF : A_0(X) \aw A_1(X)$ 
defined in chapter 5, is a non-linear version of the gradient $\nabla = \div^*$.
It measures the lack of consistency of the effective energies introduced in chapter 4.
\iii $\mu : A_1(X) \aw A_1(X)$ 
is a generalisation of the Möbius transform $\mu = \zeta^{-1}$ to higher degrees, 
this reciprocity being extended in chapter 3. 
Its effect on message-passing is discussed in chapter 5.
\iii $\div : A_1(X) \aw A_0(X)$ 
is the boundary operator of the complex $A_\bullet(X)$, defined in chapter 2. 
This construction specialises 
the general notion of simplicial groups, reviewed in chapter 1.
\ei


Each chapter begins with an introductory paragraph 
describing its content, and so does each section. 
They are briefly summarised here, as a complement 
to the full table of contents in the following pages.


\begin{enumerate}

\item {\it Homological Algebra:} 
this synthetic and self-contained chapter 
introduces elements of category theory and simplicial homology. 
It is intended for readers not yet familiar with these powerful languages,
although its short size may reasonably not substitute for a textbook. 
Homology is introduced through the categorical framework 
of simplicial objects. 

\item {\it Statistical Systems:}
this chapter develops the original point of view 
adopted throughout this work. 
Building on functoriality, it specialises abstract algebraic 
and homological constructions to our setting involved with statistics, 
by introducing a differential complex $A_\bullet(X)$ of 
local observables.
Fundamental theorems characterising its homology
are found in section 2.3.

\item {\it Combinatorics:}
this chapter introduces Dirichlet convolution and 
reviews elementary notions of incidence algebra.
Focusing on properties of the zeta transform $\zeta$ and 
Möbius inversion formulas, some of which involving the boundary operator
$\div$ of $A_\bullet(X)$, we propose an extension of $\zeta$ and its 
inverse $\mu$ to higher degrees, on which our rectified message-passing 
algorithm shall rely. 

\item {\it Energy and Information:} 
this chapter reviews the non-linear functionals 
involved in thermodynamics and information theory, 
with their associated variational principles.
Its main originality is the focus given to free and effective energies. 
The relationship of Bethe entropy with mutual informations is emphasised.
Our fundamental theorem relating solutions of the cluster variation method
with the homology of $A_\bullet(X)$ concludes section 3.3

\item {\it Message-passing and Diffusion:}
this chapter establishes the correspondence of message-passing algorithms 
with transport equations of the form $\dot u = \div \Phi(u)$ at the level 
of interaction potentials. 
Two main improvements are advised. First, finer integrators of the above
differential equation should be used, 
as BP corresponds to an explicit Euler scheme of time step 1 
and should show unstable behaviour. 
Second, 
we propose a combinatorial correction of 
BP through a degree 1 Möbius inversion,
so as to elimate redundancies in messages. 


\item {\it Geometry of Equilibria:} 
this chapter extends a well-known result on acyclic graphs 
to a wider class of {\it retractable} hypergraphs $X \incl \Part(\Om)$,  
characterising the true marginals $(p_\aa)$ as the unique equilibrium state.
We relate the appearance of singularities and bifurcations of equilibria
to spectral properties of a pseudo-laplacian operator induced by the linearised flow,
and provide with explicit examples of bifurcation on graphs with two loops. 

* * * 
\item {\it Numerical Simulations:} most structures covered in this 
thesis were implemented in javascript. 
This chapter shall exhibit some qualitative behaviour of message-passing algorithms, 
such as the influence of the time scale on stability, 
and that of the combinatorial correction of messages.
\end{enumerate}




==> intro/crystals.tex <==
There exists a true continuity between statistical models
of magnetic crystals and neural networks. 
Their main difference lies in their underlying geometry,
and the path they are related by 
leads from the distinctive symmetry of crystals, 
to the intricate connections of networks, 
through the quenched disorder of 
amorphous magnetic solids known as {\it spin glasses}. 
The perfect correspondence between microscopic interactions 
assumed by common models surely deserves more attention.
Microscopic details should however be of limited relevance
as this analogy, statistical in nature, relies on 
the emergence of collective phenomena and organised behaviour.

\input{intro/img/isingGlass.tex}

The Ising model of ferromagnetism, introduced by Lenz in 1920 for his student,
describes an assembly of magnetic dipoles or {\it spins}
with values $x_i = \pm 1$, arranged on a regular lattice. 
These spins interact only with their nearest neighbours, 
with whom they tend to be aligned. 
The total energy of the system is measured by the so-called hamiltonian 
function $H$, expressed as a sum of local interactions:
\begin{equation} \label{H-ising}
 H(x) = \sum_{ij} h_{ij}(x_i, x_j) + \sum_i h_i(x_i) 
\end{equation}
where the sums are respectively understood to run over 
edges and vertices of a finite sublattice of $\Z^d$, 
or a periodic folding of the latter, such as the  
discrete torus $(\Z / N \Z)^d$ 
describing periodic boundary conditions. 
Crystalline symmetry and the nearest-neighbour approximation 
lead to assume pairwise magnetic interactions of the form 
$h_{ij}(x_i, x_j) = - w \,x_i \, x_j$ 
so that the energy of the pair is $-w$ when $x_i = x_j$ and $+w$ otherwise,
for some coupling constant $w > 0$.
The pointwise interaction terms $h_{i}(x_i) = - b \, x_i$ 
describe the influence of an external magnetic field $b$. 
Low energies are reached when neighbouring spins are aligned, 
the external field inducing a preferred orientation.  

\input{intro/interactions.tex}

According to the principles of statistical physics, at temperature 
$T = \theta^{-1}$ the probability 
of finding the system in the configuration $x$ is given by 
the Gibbs distribution: 
\begin{equation} p_\theta(x) =  \frac {\e^{- \theta H(x)}} {Z_\theta} 
\quad\txt{where}\quad Z_\theta = \sum_x \e^{-\theta H(x)}
\end{equation} 
In the high temperature limit $\theta \to 0$, 
thermal disorder increases until $p_\theta$ becomes uniform. 
In the low temperature limit $\theta \to +\infty$ 
the system freezes into the minimal energy state, all spins aligned
with $b$. 
The spontaneous magnetisation $\E_\theta[x_i]$ measures the self-ordering 
of the system in the limits $b \to 0^\pm$, 
and the existence of a phase transition 
at the Curie temperature $T = T_c$, 
under which the material becomes a permanent magnet
expresses a sharp variation of this quantity with respect to $\theta$ at $1 / T_c$. 
The steepness becomes a discontinuity in the thermodynamic limit 
where the number of atoms goes to infinity, 
and the theoretical modelling of such phase transitions is 
the challenge faced by statistical physics\footnote{
    Let us only mention that an analytical solution of the Ising model for $d = 2$ 
    was first proven by Onsager in 1944, while little is known for $d = 3$. 
    Despite its apparent simplicity, 
    the model is rich enough to capture phase transitions 
    and resist a century of exploration.
}. 

In contrast with ferromagnetic crystals, spin glasses
present a quenched disorder,
which reflects their irregular structure and persists at low temperatures\footnote{
    Their strange magnetic behaviour was first noticed in diluted alloys of 
    magnetic manganese atoms inside non-magnetic copper. Dipole interactions
    being mediated by the conductor's free electrons, the sign and intensity of the 
    couplings vary faster than the interatomic length and appear random.   
}, 
similar to that of amorphous solids.  
This intrinsic disorder translates into a randomisation 
of magnetic couplings $w_{ij}$, varying in sign and intensity depending on 
the bond. Replacing pairwise interactions by $h_{ij}(x_i, x_j) = - w_{ij}(x_i, x_j)$
in equation \ref{H-ising} 
yields the so-called Edwards-Anderson model, 
where atoms still lie on a regular lattice.
The Sherrington-Kirkpatrick model lets the sum run over all possible pairs $i,j$
and consists of a mean-field approximation of the former, atoms being joined  
in a fully connected graph. 
Such materials exhibit very peculiar behaviour, 
among which are strong hysteresis phenomena and 
a form of ergodicity breaking: the system never reaches minimal energy equilibrium 
due to a very complex energy landscape. 

The interest of spin glass theory however goes far beyond condensed matter physics, 
as pairwise magnetic interactions are equivalent to usual 
models of neuronal activity.
In this correspondence, 
neuron $i$ is in the state $x_i = -1$ when it is at rest, 
and in the state $x_i = +1$ when it is firing at maximal rate, 
while intermediate firing rates are naturally described by 
a convex combination or binary probability density $q_i(x_i)$. 
The firing rate $r_i = q_i(+1)$ of a neuron varies smoothly as a function of its 
membrane potential, so that it is often modeled by the so called 
<<sigmoid>> neuron: 
\begin{equation} r_i = \sigma_\lambda \Big( \sum_{j} w_{ij} r_j + b_j \Big) 
\quad \txt{with} \quad
\sigma_\lambda(t) = \frac 1 {1 + \e^{- \lambda t}}
\end{equation}
From the magnetic perspective, the probability distribution of $x_i$ 
given the state of its neighbours is given by: 
\begin{equation} p\big(x_i \st (x_j)_{j \neq i} \big)  \end{equation}

Firing rates may 

\ref{tab:interactions}


Hopfield networks similarly consist of an assembly of binary variables.

\cite{Hopfield-82, Amit-87}

\input{intro/img/boltzmannMachines.tex}


\input{intro/img/phases.tex}



==> intro/img/neuron.tex <==
Firing rate versus membrane voltage for a typical neuron (solid line),
dropping to 0 for large negative potentials and saturating
for positive potentials. 



==> intro/img/phases.tex <==
\begin{figure}[t]
    \sbox0{\includegraphics[width=0.85\textwidth]{img/phases.png}}
\begin{center}
\begin{minipage}{\wd0+0\textwidth}
\centering
\usebox0
\caption{
    Phase transitions in the Hopfield model. 
    Left: loss of retrieval performance 
    with memory load, (a) Hopfield 
    and (b) Amit.  
    Right: (c) phase diagram and (d) a low-temperature detail, 
    Amit et. al.
}
\end{minipage}
\end{center}
\end{figure} 


==> intro/interactions.tex <==
\begin{table}[t]
\vspace{0.5cm}
\begin{center}
{\renewcommand{\arraystretch}{1.4} 
    \setlength\abovedisplayskip{-6pt}
    \setlength\belowdisplayskip{0pt}
    \begin{tabular}
{|*2{>{\centering\arraybackslash}p{.3\textwidth}|}}
%{| C{4cm} | C{4cm} |}
    \hline
    pairwise interaction & external field \\
    \hline
    $h_{ij}(x_i, x_j) = -w_{ij}\, x_i\, x_j$ &
    $h_i(x_i) = -b_i\, x_i$ \\
    \hline 
$$ w_{ij} \cdot \left(\begin{array}{rr} -1 & 1 \\ 1 & -1 \end{array}\right) $$ 
    &
$$ b_i \cdot \left(\begin{array}{r} -1 \\ 1 \end{array}\right) $$ 
    \\
        \hline
    \end{tabular}
}

    \caption{Magnetic interactions of binary spins.}
    \label{tab:interactions}
\end{center}
\end{table}



==> intro/intro.tex <==
Factor graphs $\eqvl$ hypergraphs describe the structure of a Markov random field:
\begin{equation} p_\Om(x_\Om) = \frac{1}{Z_\Om} \prod_{\aa \incl \Om} f_\aa(x_\aa) \end{equation}
Two collections of factors $(f_\aa) \sim (f'_\aa)$ are said 
{\it homologous} when $\prod_\aa f_\aa \simeq \prod_\aa f'_\aa$ 
up to a scaling factor,
{\it i.e.} they both provide a factorisation of the same global probability
distribution $p_\Om$. 
The normalisation factor $Z_\Om$ being intractable, the strategy of $\BP$ 
is to approximate the marginals $(p_\aa)$ of $p_\Om$ by finding a collection 
of beliefs $(q_\aa)$ satisfying the {\it consistency} condition: 
\begin{equation} q_\bb(x_\bb) = \sum_{y \in E_{\aa \setminus \bb}} q_\aa(x_\bb, y) \end{equation}
deriving from homologous factors $(f'_\aa) \sim (f_\aa)$ according to a 
local analog of the equation defining $p_\Om$:
\begin{equation} q_\aa(x_\aa) = \frac{1}{Z_\aa} \prod_{\bb \incl \aa} f'_\bb (x_\bb) \end{equation}
The fundamental property of message-passing algorithms is to explore  
a homology class of factors. 
Various message-passing algorithms exist, all associated to different kinds 
of approximations for computational purposes. These approximations 
affect their stationarity, hence the consistency condition 
should be replaced accordingly.

\section*{Markov Random Fields and Graphical Models}

Denote by $p \in {\cal M}(X)$ positive
Markov random fields subordinate to the hypergraph $X \incl \Part(\Om)$.
Alternatively represent $X$ by a factor graph, 
although this hides combinatorial structures.

Then $p = \prod_\aa f_\aa \in {\cal M}(X)$ is a homology class of factors, we write
$(f_\aa) \sim (f'_\aa)$ whenever their products coincide.
The logarithm and the zeta transform shall induce a diffeomorphism: 
\begin{equation} {\cal M}(X) \simeq A_0(\Xint) / \divint A_1(X) \end{equation} 
That is, homology takes place at the level of interaction potentials.

If $X \incl Y$ then ${\cal M}(X) \incl {\cal M}(Y)$. 
Quotient map $\Om \aw \Om /{\sim}$ induces $X \aw X/{\sim}$ and 
${\cal M}(X) \aw {\cal M}(X/{\sim})$, 
which corresponds to grouping factors together. 
For instance when $X$ is layered along $\Om = \Om_0 \sqcup \dots \sqcup \Om_n$,
the quotient map sends $p$ to a Markov chain.  

When $X$ is retractable, e.g. is a chain or a tree, 
we have a canonical factorisation: 
\begin{equation} p = \prod_\aa p_\aa^{c_\aa} \end{equation}
where $p_\aa$ denotes the marginal of $p$ on $\aa$. 
The above formula is not true in general, and fails as soon as $X$ has loops.


\section*{From Crystals to Neural Networks}

Ising model, Spin glasses, Hopfield networks, Boltzmann machines. 

Deep neural networks as approximate Markov chains? 

\section*{Bayesian Learning and Message-passing Algorithms}

Maximise over parameters $h$ the log-likelihood of observed data 
$\bar x \in (E_\Om)^N$:
\begin{equation} {\cal L}(\bar x, h) = \frac{1}{N} \sum_{i = 1}^N \log 
p(x^{(i)} \st h) \end{equation}
For fully observed models $\bar x = \bar x_\Om$ and a parametrisation 
$p_\Om \simeq \prod_\aa \e^{-h_\aa}$ the log-likelihood is given by:
\begin{equation} {\cal L}(\bar x, h) = - \sum_\aa \bar \E^\aa[h_\aa] 
- \log Z_\Om(h) \end{equation}
where $\bar \E^\aa$ denotes expectation with respect to the empirical marginal. 
Letting $H_\Om = \sum_\aa h_\aa$ denote the global hamiltonian and 
$\Fh^\Om(H_\Om) = - \log \sum \e^{-H_\Om}$ denote the total free energy, 
the log-likelihood rewrites: 
${\cal L}(\bar x, h) = \Fh^\Om(H_\Om) - \bar \E^\Om[H_\Om]$.
Its variations are given by:
\begin{equation} \der{\cal L}{h_\aa} = p_\aa - \bar p_\aa \end{equation} 
Denoting by $p_\aa = \Sigma^{\aa\Om} \e^{-H_\Om}$ the model marginal 
and by $\bar p_\aa$ the empirical marginal. 
Belief propagation allows to estimate $p_\aa$ to perform gradient ascent on $\cal L$.

Partial observations on variables $\bord \Om \incl \Om$ with 
$\bar y \in (E_{\bord \Om})^N$:  
\begin{equation} {\cal L}(\bar y, h) 
= \frac 1 N \sum_{i = 1}^N \log p(y^{(i)} \st h) \end{equation}
Writing $- \log p_{\bord \Om} = \Fh^\Om(H_\Om \st \bord \Om) - \Fh^\Om(H_\Om)$ 
with $H_\Om = \sum_\aa h_\aa$ we get: 
\begin{equation} - \der {\cal L} {h_\aa} 
= \bar \E^{\bord \aa} \big[ \E^\aa[h_\aa \st \bord \aa] \big]
- \E^\aa[h_\aa] \end{equation}
where $\bar \E^{\bord \aa}$ denotes expectation with respect to the empirical 
marginals. 
Determination of the model marginals allow for gradient descent on $-{\cal L}$,
and yield both $\E^\aa[-\st \bord \aa]$ and $\E^\aa[-]$. 

{\bf N.B.} In a restricted Boltzmann machine, the hidden nodes are conditionally 
independent given the state of the visible ones. 
Hence the so-called <<positive-phase>> is easily computed through: 
\begin{equation} p(x_{\mathring \Om} \st y) 
= \prod_{i \in \mathring \Om} p(x_i \st y) 
\end{equation}
However the <<negative-phase>> still requires approximate marginals, 
which yield the <<positive-phase>> in the general case. 


